A Novel Technique for Evidence based Conditional Inference in Deep Neural Networks via Latent Feature Perturbation

Auxiliary information can be exploited in machine learning models using the paradigm of evidence based conditional inference. Multi-modal techniques in Deep Neural Networks (DNNs) can be seen as perturbing the latent feature representation for incorporating evidence from the auxiliary modality. However, they require training a specialized network which can map sparse evidence to a high dimensional latent space vector. Designing such a network, as well as collecting jointly labeled data for training is a non-trivial task. In this paper, we present a novel multi-task learning (MTL) based framework to perform evidence based conditional inference in DNNs which can overcome both these shortcomings. Our framework incorporates evidence as the output of secondary task(s), while modeling the original problem as the primary task of interest. During inference, we employ a novel Bayesian formulation to change the joint latent feature representation so as to maximize the probability of the observed evidence. Since our approach models evidence as prediction from a DNN, this can often be achieved using standard pre-trained backbones for popular tasks, eliminating the need for training altogether. Even when training is required, our MTL architecture ensures the same can be done without any need for jointly labeled data. Exploiting evidence using our framework, we show an improvement of 3.9% over the state-of-the-art, for predicting semantic segmentation given the image tags, and 2.8% for predicting instance segmentation given image captions.

==> sections/acko.tex <==
\section{Acknowledgements}\label{sec:acknowledgements}
 


==> sections/algo_v0.tex <==


\section{Our Approach}
In this section. we present our approach for incorporating test time evidence in a DNN. The Bayesian network which models the dependency between random variable $X$ (input), $Y$ (primary output) and $A$ (auxiliary output) is shown in figure~\ref{fig:bayesian_network}. Given the evidence $A=e$ at test time, we are interested in computing
the probability $P(Y|X=x, A=e)$.  In the light of this observation $e$, we would like to perturbing input $x$ to $\hat{x}$ such that $\hat{x}$ contains the information available in the evidence $e$ i.e., $P(Y|X=x, A=e)=P(Y|X=\hat{x})$.  One way to obtain $\hat{x}$ is by maximizing the probability of observing $A=e$ i.e., $\hat{x}= \argmax_{x} P(A=e|X=x)$. Now once we have this evidence specific input $\hat{x}$, we can calculate the $P(Y|X=\hat{x})$. We have modeled the probabilities $P(Y|X=x)$ and $P(A|X=x)$ using DNNs and in the next section we show how to use back-propagation to obtain $\hat{x}$.


\begin{figure}[t]
	\centering
	\subfigure{\includegraphics[width=0.5\linewidth,height=0.5\linewidth]{./figures/bayesian_network.pdf}}
	\caption{Bayesian network modeling the dependency between $X$ (input), $Y$ (primary output) and $A$ (auxiliary output). $X$ and $A$ are observed variables at the test time and are shown in gray. }
	\label{fig:bayesian_network}
\end{figure}







\section{Framework for Back-propagating Evidence}\label{sec:model}

In this section, we present our approach for boosting up the accuracy of a given task of interest by incorporating evidence. Our solution employs a generic MTL~\cite{ruder2017overview} based architecture which consists of a main (primary) task of interest, and another auxiliary task whose desired output (label) represents the evidence in the network. The key contribution of our framework is its ability to back-propagate the loss on the auxiliary task during prediction time, such that weights are re-adjusted to match the output of the auxiliary task with given evidence. In this process, as we will see, the shared weights (in MTL) also get re-adjusted producing a better output on the primary task. This is what we refer to as back-propagating evidence through the network (at prediction time). We note that though we describe our framework using a single auxiliary task to keep the notation simple, it is straightforward to extend this to a setting with more one than auxiliary task (and associated evidence at prediction time).
%\paragraph*{Model}

\begin{figure}[t]
	\centering
	\subfigure{\includegraphics[width=\linewidth]{./figures/model_architecture.pdf}}
	\caption{Model Architecture for Multi-task learning (MTL)}
	\label{fig:model_architecture}
\end{figure}

\begin{figure}
	\begin{center}
		\centering
		\subfigure{\includegraphics[width=\linewidth]{./figures/train_test_loss.pdf}}
		\caption{Loss propagation at train and prediction time}
		\label{fig:loss_propagation}		
	\end{center}	
	%\hfill
\end{figure}



\subsection{Background on MTL}
\paragraph*{Notation}
We will use $P$ to denote the primary task of interest. Similarly, let $A$ denote the auxiliary task in the network. Let $(x^{(i)},y^{(i)},a^{(i)})$ denote the $i^{th}$ training example, where $x^{(i)}$ is input feature vector, $y^{(i)}$ is desired output (label) of the primary task, and $a^{(i)}$ denotes the desired output (label) of the auxiliary task. Correspondingly, let $\hat{y}^{(i)}$ and $\hat{a}^{(i)}$ denote the output produced by the network for the primary task and auxiliary tasks, respectively. 

\paragraph*{Model} Figure~\ref{fig:model_architecture} shows the MTL based architecture~\cite{ruder2017overview} for this set-up. There is a common set of layers shared between the two tasks, followed by the task specific layers. $z$ represents the common hidden feature representation fed to the two task specific parts of the architecture. For ease of notation, we will refer to the shared set of layers as {\em trunk}.
% and the two task specific set of layers as \em{branch_M}, \em{branch_S}, respectively. 

The network has three sets of weights. First, there are weights associated with the trunk denoted by $W_{zx}$. $W_{yz}$ and $W_{az}$ are the sets of weights associated with the two task specific branches, respectively. The total loss $\LS^{T}(\cdot)$ is a function of these weight parameters and can be defined as:
\begin{equation}
%\label{eq:loss_training}
\LS_{T}(\cdot)=\sum_{i=1}^{m} \left(\LS_{P}(y^{(i)},\hat{y}^{(i)})\right)+ \lambda \sum_{i=1}^{m} \left(\LS_{A}(a^{(i)},\hat{a}^{(i)})\right) \nonumber
\end{equation}
Here, $\LS_{P}(\cdot)$ and $\LS_{A}(\cdot)$ denote the loss for the primary and auxiliary tasks, respectively.  $\lambda$ is the importance weight for the auxiliary task. The sum is taken over the $m$ examples in the training set. $\LS_{P}$ is a function of the shared set of weights $W_{zx}$, and the task specific weights $W_{yz}$. Similarly, and $\LS_{A}$ is a function of the shared weights $W_{zx}$ and task specific weights $W_{az}$, respectively.
%$LS_{total}$ depends on the weight parameters.

\paragraph*{Training}
The goal of training is to find the weights which minimize the total loss over the training data. Using the standard approach of gradient descent, 
the gradients can be computed as follows:
\begin{enumerate}
\item $\nabla_{W_{yz}} \LS(\cdot) = \sum_{i=1}^{m} \nabla_{W_{yz}} \LS_P(\cdot)$
\item $\nabla_{W_{az}} \LS(\cdot) = \sum_{i=1}^{m} \nabla_{W_{az}} \LS_A(\cdot)$
\item $\nabla_{W_{zx}} \LS(\cdot) = \sum_{i=1}^{m} \nabla_z \LS_P(\cdot) \nabla_{W_{zx}}(z) + \lambda \sum_{i=1}^{m} \nabla_z \LS_A(\cdot) \nabla_{W_{zx}} (z)$
\end{enumerate}

Note that the weights in the task specific branches, i.e., $W_{yz}$ and $W_{az}$, can only affect losses defined over the respective tasks (items 1 and 2 above). On the other hand, weights $W_{zx}$ in the trunk affect the losses defined over both the primary as well as the auxiliary tasks. Next, we describe our approach of back-propagating the loss over the evidence.
%\item 

\subsection{Our Approach - Prediction}
%\paragraph*{Prediction}
During test time, we are given additional information about the output of the auxiliary task. Let us denote this by $e$ (evidence) to distinguish it from the auxiliary outputs during training time. Then, for the inference, instead of directly proceeding with the forward propagation, we instead first decide to adjust the weights of the network such that the network is forced to match the evidence $e$ on the auxiliary task. Since the two tasks are correlated, we expect that this process will adjust the weights of the network in a manner such that resolving the ambiguity over the auxiliary output will also result in an improved prediction over the primary task of interest.

This feat can be achieved by defining a loss in terms of $\LS_A(\hat{a},e)$ and then back-propagating its gradient through the network. Note that this loss only depends on the set of weights $W_{az}$ in the auxiliary branch, and the weights $W_{zx}$ in the trunk. In particular, the weights $W_{yx}$ remain untouched during this process. Finally, we would also like to make sure that our weights do not deviate too much from the originally learned weights. This is to avoid over-fitting over evidence. This can be achieved by adding a two-norm based regularizer which discourages weights which are far from the originally learned weights. The corresponding weight update equations can be derived using the following gradients:
\begin{enumerate}
\item $\nabla_{W_{az}} \LS_{Test}(\cdot) = \nabla_{W_{az}} \LS_A(\hat{a},e) + \alpha||W_{az}-W^*_{az}||^2$
\item $\nabla_{W_{zx}} \LS_{Test}(\cdot) = \nabla_z \LS_A(\hat{a},e) \nabla_{W_{zx}}(z) + \alpha||W_{zx}-W^*_{zx}||^2 $ 
\end{enumerate}

Here, $W_{az}^{*}$ and $W_{zx}^*$ denote the weights learned during training and $\alpha$ is the regularization parameter. Note that these equations are similar to those used during training (item 2 and 3), with the differences that (1) The loss is now computed with respect to the single test example (2) Effect of the term dependent on primary loss has been zeroed out. (3) A regularizer term has been added. In our experiments, we also experimented with early stopping instead of adding the norm based regularizer.

Algorithm~\ref{algo:weight_update} describes our algorithm for weight update during test time, and Figure \ref{fig:loss_propagation} explains it pictorially. Once the new weights are obtained, they can be used in the forward propagation to obtain the desired value $\hat{y}$ on the primary task. %It is important to note that the weight update in our framework at the test time are done for a particular sample and do not persist for the next example. 

\begin{algorithm}[t]
	\begin{algorithmic}[1]
		\INPUT $\x$ (input), $e$: evidence 
		%\INPUT $\eta$ \Comment{Learning rate}
		%\INPUT $T$ \Comment{Iterations}
		%\INPUT $\Delta$ \Comment{Loss function}
		\INPUT $\eta$ (Learning rate), $T$ (Iterations),
		\INPUT $W^{*}_{az}$, $W^{*}_{zx}$: Originally trained weights 
		\OUTPUT $W_{az}, W_{zx}$   
		%\Comment{predicted output corresponding to $\x$}
		
		\For {$t \in \{1,\dots,T\}$};
		\State Calculate the loss $\LS_{test}(\hat{a},e)$ over evidence
		\State Compute $\nabla_{W_{az}} \LS_{test}(\cdot)$ and $\nabla_{W_{zx}} L_{test}(\cdot)$, using back-propagation 
		%\frac{\partial \LS^{test}(\cdot)}{\partial \z} = \sum_{i=1}^{m} \lambda_{\TS_{i}}   \frac{\partial \LS_{\TS_{i}}(y_{\TS_{i}},\hat{y}_{\TS_{i}})}{\partial \z}$
		\State Update $W_{az}$ and $W_{zx}$ using gradient descent rule
		%Back-Propagate the gradient of test loss ($\LS^{test}$) 
		%\State Update the parameters of network.
		\EndFor
		\State Return the newly optimized weights
		
	\end{algorithmic}
	\caption{weight update algorithm}
	\label{algo:weight_update}
\end{algorithm}



==> sections/background.tex <==
\section{Background on MTL}\label{sec:background}
Our solution employs a generic MTL~\cite{ruder2017overview} based architecture which consists of a main (primary) task of interest, and another auxiliary task whose desired output (label) represents the evidence in the network. In this section, we present the background on MTL which we will build on in Section~\ref{sec:approach}.
\paragraph*{Notation}
We will use $P$ to denote the primary task of interest. Similarly, let $A$ denote the auxiliary task in the network. Let $(x^{(i)},y^{(i)},a^{(i)})$ denote the $i^{th}$ training example, where $x^{(i)}$ is input feature vector, $y^{(i)}$ is desired output (label) of the primary task, and $a^{(i)}$ denotes the desired output (label) of the auxiliary task. Correspondingly, let $\hat{y}^{(i)}$ and $\hat{a}^{(i)}$ denote the output produced by the network for the primary task and auxiliary tasks, respectively. 

\paragraph*{Model} Figure~\ref{fig:model_architecture} shows the MTL based architecture~\cite{ruder2017overview} for this set-up. There is a common set of layers shared between the two tasks, followed by the task specific layers. $z$ represents the common hidden feature representation fed to the two task specific parts of the architecture. For ease of notation, we will refer to the shared set of layers as {\em trunk}.
% and the two task specific set of layers as \em{branch_M}, \em{branch_S}, respectively. 

The network has three sets of weights. First, there are weights associated with the trunk denoted by $W_{zx}$. $W_{yz}$ and $W_{az}$ are the sets of weights associated with the two task specific branches, respectively. The total loss $\LS^{T}(\cdot)$ is a function of these weight parameters and can be defined as:
\begin{equation}
%\label{eq:loss_training}
\LS_{T}(\cdot)=\sum_{i=1}^{m} \left(\LS_{P}(y^{(i)},\hat{y}^{(i)})\right)+ \lambda \sum_{i=1}^{m} \left(\LS_{A}(a^{(i)},\hat{a}^{(i)})\right) \nonumber
\end{equation}
Here, $\LS_{P}(\cdot)$ and $\LS_{A}(\cdot)$ denote the loss for the primary and auxiliary tasks, respectively.  $\lambda$ is the importance weight for the auxiliary task. The sum is taken over the $m$ examples in the training set. $\LS_{P}$ is a function of the shared set of weights $W_{zx}$, and the task specific weights $W_{yz}$. Similarly, and $\LS_{A}$ is a function of the shared weights $W_{zx}$ and task specific weights $W_{az}$, respectively.
%$LS_{total}$ depends on the weight parameters.

\paragraph*{Training}
The goal of training is to find the weights which minimize the total loss over the training data. Using the standard approach of gradient descent, 
the gradients can be computed as follows:
\begin{enumerate}
\item $\nabla_{W_{yz}} \LS(\cdot) = \sum_{i=1}^{m} \nabla_{W_{yz}} \LS_P(\cdot)$
\item $\nabla_{W_{az}} \LS(\cdot) = \sum_{i=1}^{m} \nabla_{W_{az}} \LS_A(\cdot)$
\item $\nabla_{W_{zx}} \LS(\cdot) = \sum_{i=1}^{m} \nabla_z \LS_P(\cdot) \nabla_{W_{zx}}(z) + \lambda \sum_{i=1}^{m} \nabla_z \LS_A(\cdot) \nabla_{W_{zx}} (z)$
\end{enumerate}

Note that the weights in the task specific branches, i.e., $W_{yz}$ and $W_{az}$, can only affect losses defined over the respective tasks (items 1 and 2 above). On the other hand, weights $W_{zx}$ in the trunk affect the losses defined over both the primary as well as the auxiliary tasks. Next, we describe our approach of back-propagating the loss over the evidence.
%\item 

\begin{figure}[t]
	\centering
	\subfigure{\includegraphics[width=\linewidth]{./figures/model_architecture.pdf}}
	\caption{Model Architecture for Multi-task learning (MTL)}
	\label{fig:model_architecture}
\end{figure}


==> sections/related_v0.tex <==
\section{Related Work}\label{sec:relatedwork}

As argued earlier, though our architecture may seem similar in style to existing work trying to boost up the performance of the primary task based on auxiliary tasks~\cite{liang2015semantic, bingel2017identifying, romera2012exploiting}, the key difference is 
%that whereas
%lies in the fact that  
%using MTL. The key difference is 
%whereas 
that, while, the earlier works exploit the use of correlated tasks only during the training process, we in addition, employ a Bayesian formulation to modify the internal feature representation during prediction time so that probability of outputting the observed auxiliary label(s) is maximized.
%focus on back-propagating the available (instance specific) evidence during prediction time as well. This is an important conceptual difference and can result in significant improvements by exploiting additional information as shown by our experiments.

We would also like to differentiate our work from that of posterior inference with priors. While priors can be learned for sample distributions, our work suggests conditional inference in the presence of sample specific evidence. Similarly, posterior regularization technique~\cite{ganchev2010posterior} changes the output distribution directly, albeit, only based on characteristics of the underlying data statistics. No sample specific evidence is used.

Another closely related research area is multi-modal inference~\cite{rosenfeld2018priming, kilickaya2016leveraging, cheng2014imagespirit} which also incorporates additional features from auxiliary information. While this does effectively incorporate evidence at prediction time in the form of additional features, but practically speaking, designing a network to take additional information from a highly sparse information source is non-trivial \footnote{For example, in one of our experiments we show the semantic segmentation conditioned upon image level tags as given by an image classification task. It is easy to see that designing an MTL based DNN architecture for semantic segmentation and image classification is not difficult. On the other hand, designing a network which takes a single image label and generates features for merging with RGB image features seems non-trivial.}. However, the strongest argument in support of our framework is its ability to work even when only single set of annotations are available. It is possible to train our architecture even when we have dataset containing either primary or auxiliary annotations. On the other hand, multi-modal input based architecture would require a dataset containing both the annotations at the same time. This greatly restricts its applicability. Note that the argument extends to test time also. At test time, if auxiliary information is unavailable our framework can fall back to regular predictions, while architecture with multi-modal input will fail to take-off.

\begin{comment}
there are some important differences: 
\begin{enumerate}
	\item In a typical multi-modal framework side information is a strict requirement. However, our framework can naturally fall back to regular predictions if the evidence is not available for particular sample(s). The only alternative to using our framework is training two separate networks: one MTL framework with joint learning of two kind of tasks, and another multi-modal framework with two inputs. Then, depending upon whether an evidence is available at test time, one resorts to using one of the two networks. Our framework can work with only a single network of former kind, without any additional significant overheads.
	\item Even if training two separate networks, as suggested above, is theoretically possible, designing a network to take additional information from highly sparse information source is non-trivial. For example, in one of our experiments we show the semantic segmentation conditioned upon image level tags as given by an image classification task. It is easy to see that designing an MTL based DNN architecture for semantic segmentation and image classification is not difficult. On the other hand, designing a network which takes a single image label and generates features for merging with RGB image features seems non-trivial. 
\end{enumerate}
\end{comment}

Some recent works~\cite{pathak2015constrained, xu2017semantic, marquez2017imposing} have proposed constraining the output of DNN, to help regularizing the output and reduce the amount of training data required. While all these works suggests constraints during training, our approach imposes the constraints both at the train and inference time.

We note that our framework is similar in spirit to another contemporary work by Lee et al. \cite{lee2017enforcing}, who have also proposed to enforce test time constraints on a DNN output. However, while their idea is to enforce `prior deterministic constraints' arising out of natural rule based processing, our framework is inspired from using any easily available and arbitrary type of auxiliary information. Our framework can be used together with theirs, as well as, is more generalizable due to lack of requirement of using the constraints on the output of the same stream. 

\begin{comment}

\subsection{Multitask learning}
Our framework is based on one of the popular approaches to MTL in deep networks known as hard parameter sharing~\cite{caruana1995learning}. In this approach, all the tasks share some hidden layers of the DNN followed by task-specific layers.
Since these tasks share a joint representation through the shared layers,  it helps in preventing over-fitting\cite{maurer2006bounds}, even when the amount of training data is less for each task. There is also another set of work in which a set of main tasks is augmented by a related set of auxiliary task~\cite{alonso2017multitask,liang2015semantic,bingel2017identifying,romera2012exploiting}. Our framework enjoys all the benefits of MTL, besides being able to use information from the auxiliary task at inference time as well. 

\subsection{Constraining the Output of DNN}
There are many applications like image segmentation, medical imaging, machine translation, speech recognition, etc. where labeling data is expensive and difficult. So researchers are currently focussing on putting constraints on the output of DNN, as it reduces the need for labeled training data and increases the quality of prediction. This gave rise to the whole area of weak supervision. ~\cite{pathak2015constrained} does weakly supervised semantic segmentation by training only from image-level labels and also applies object size constraints on the segmentation output. Both the constraints are incorporated in the training procedure through a series of linear constraints. There are also works in which researchers enforce the constraints by suitably designing the loss function ~\cite{xu2017semantic,kervadec2018constrained}. All of these approaches apply soft constraints on the output as there is no guarantee that the constraints will be satisfied. Since the constraints are applied only once on the whole data, it makes designing such constraints difficult and also requires significant domain knowledge. In our approach, we apply the constraints at training time by learning the main and auxiliary tasks jointly. We also use the auxiliary information for each of the examples at inference time to constraint the predicted output of the main task. ~\cite{marquez2017imposing} studied the effect of applying hard constraints and found out that soft constraints give better results at significantly less computational cost. There are other works which puts logical constraints on the output of DNN such as in ~\cite{hu2016harnessing,rocktaschel2015injecting,donadello2017logic,stewart2017label}. 

\subsection{Probabilistic Graphical Models}

\end{comment}



==> sections/results_instance_seg_bak.tex <==
\subsection{Instance Segmentation}
\label{sec:instance_seg}

Next, we present our experimental evaluation on a multi-modal task of object instance segmentation given textual description of the image. In an instance segmentation problem the goal is to detect and localize individual objects in the image along with segmentation mask around the objects. In our framework, we model instance segmentation as the primary task and image captioning as the auxiliary. Arguably, instance segmentation is more challenging than semantic segmentation, and incorporating caption information also seems significantly harder due to its frequent noisy and incomplete nature. We speculate this to be the reason behind lack of any prior noticeable work using textual description for improving instance segmentation. 

\myparagraph{Our Implementation} 
%
Our MTL based architecture is shown is Figure~\ref{fig:instance-seg-proposed-arch}. We take Mask R-CNN~\cite{he2017mask}, a state-of-the-art instance segmentation approach, and combine it with the LSTM decoder from the captioning generator ``Show, Attend and Tell''(SAT)~\cite{xu2015show} within our framework. We use publicly available implementation of Mask R-CNN \cite{mrcnn-code} (with ResNeXt-152 \cite{xie2017aggregated} backbone), as well as SAT \cite{sat-code}. We initialize our primary network with the pre-trained weights of the Mask R-CNN from \cite{mrcnn-weights}, and fine-tune with caption decoder (secondary task) using our MTL architecture. Early stopping iterations parameter was set at 2, and $\alpha$ parameter was set to 100. We have used Adam optimizer with a learning rate of $5*10^{-6}$ at test time.

\begin{figure}[t]
	\centering
	\subfigure{\includegraphics[width=\linewidth]{./figures/instance-seg-proposed-arch.pdf}}
	\caption{Our framework for instance segmentation using Mask-RCNN and LSTM based caption generator to use textual descriptions of an image at test time.}
	% Note that BB refers to bounding box.}
	\label{fig:instance-seg-proposed-arch}
\end{figure}

\myparagraph{Comparison} 
%
The table on the right below shows our comparison with various baselines. 
\setlength{\columnsep}{5pt}%
\setlength{\intextsep}{5pt}%
\setlength{\tabcolsep}{2pt}
\begin{wraptable}{r}{0.7\linewidth}
	\centering
	\begin{tabular}{llllll}
		\toprule[1.5pt]
		\textbf{Method} & \textbf{AP} & \textbf{AP\textsubscript{0.5}}&\textbf{AP\textsubscript{S}} & \textbf{AP\textsubscript{M}}& \textbf{AP\textsubscript{L}}\\
		\midrule
		MRCNN &  39.8 & 63.5  & 39.4 & 69.0  &  80.0 \\ 
		MMT &  39.9 & 63.6  & 39.2 & 69.2  &  79.8 \\ 
		MM & ?? & ?? & ?? & ?? & ?? \\
		Ours-L2 &  \textbf{40.5} & \textbf{64.6} & \textbf{40.2} & \textbf{70.0}  & 81.2\\ 
		Ours-ES &  \textbf{40.5} &  \textbf{64.6} & 40.1 & \textbf{70.0}  & \textbf{82.1}    \\
		\bottomrule[1.5pt]
	\end{tabular}
\end{wraptable}
MRCNN is the original Mask RCNN instance segementation model and MMT is the same model trained using MTL. MM refers to the multi modal network which merges SAT features into the last layer of the MRCNN. We compare with two versions of approach with early stopping (ES) and L2 norm regularizers. Our attempts with pruning based approaches did not yield any gain in this case, since learning the label set to be pruned (using captions) turned out to be quite difficult. We report our results on the validation set of MS-COCO \cite{lin2014microsoft}. We use AP (average precision) as our evaluation metric, and evaluate at AP\textsubscript{0.5} (IoU threshold of 0.5). AP\textsubscript{L}, AP\textsubscript{M},AP\textsubscript{S} represent AP\textsubscript{0.5} values for large, medium and small objects, respectively.

\myparagraph{Results on Small Objects}
%
The table on the results presents the comparison for detecting various objects 
\setlength{\columnsep}{5pt}%
\setlength{\intextsep}{5pt}%
\setlength{\tabcolsep}{3pt}
\begin{wraptable}{r}{0.75\linewidth}
	\centering
	\begin{tabular}{lllllll}
		\toprule[1.5pt]
		\textbf{Type} & \multicolumn{3}{c}{\textbf{MMT}} & \multicolumn{3}{c}{\textbf{Ours-ES}} \\
		\midrule
		& \textbf{P}           & \textbf{R}         & \textbf{F1}          & \textbf{P}            & \textbf{R}           & \textbf{F1}           \\
		\midrule
		All           & 86.1  &  51.7 &  64.6   &   83.6 &  54.6 &  66.1       \\
		Small          & 80.6  & 29.8 &  43.5  &  77.9 & 31.9 & 45.3        \\
		Medium        & 86.6  & 61.3 &  71.8  & 83.9 &  64.5 &  72.9       \\
		Large         & 89.8 & 76.5 &  82.6 &  87.6 & 80.6 &  84.0   \\
		\bottomrule[1.5pt]   
	\end{tabular}
\end{wraptable}
in terms of precision (P), recall (R) and f-measure (F1), at 0.5 IoU and 0.9 confidence threshold. 
We observe the maximum gain for small objects using our method, which makes sense since a large number of them remain undetected in the original model. Careful analysis revealed that ground truth itself has inconsistencies missing several smaller objects, undermining the actual gain obtained by our approach. We give the detailed analysis in the supplementary material.

\begin{figure}[t]
	\centering
	\subfigure{\includegraphics[width=0.99\linewidth]{./figures/instance-seg-vis-results_main.pdf}}
	\caption{Comparative results for instance segmentation given image description. Text at the top top of each column, shows the given image caption. Our approach is able to discover new objects (and their segmentation) which were missed earlier.}
	\label{fig:instance-seg-vis-results-main}
\end{figure}

\myparagraph{Visual Results}
%
Figure \ref{fig:instance-seg-vis-results-main} show visual output from our framework. We note that our algorithm can detect newer objects, as well as detect additional objects of the same category. At times it is able to detect the objects which are not even mentioned in the caption, but are merely correlated with the caption.  

==> sections/results_miscellaneous.tex <==
<<<<<<< HEAD
=======
\subsection{Using Multiple Evidence Simultaneously}

We have conducted experiments on using multiple types of auxiliary information simultaneously in our instance segmentation setup. In addition to using captions as auxiliary information, we added image tags as the second source of auxiliary information. Figure~\ref{fig:instance-seg-captions-tags-proposed-arch} describes our proposed MTL architecture in detail. Here we take Mask R-CNN, a state-of-the-art instance segmentation network to generate image level features. Using these intermediate features an LSTM based decoder from the state-of-the-art captioning generator ``Show, Attend and Tell''(SAT)~\cite{xu2015show} is used to generate the captions and a multi-class classifier is designed to generate image level tags. The model was trained in a multi-task setting (one primary and two auxiliary). The evidence over the two auxiliary tasks was propagated simultaneously during test time. Table~\ref{table:instance_segmentation_caption_tags_comparison} shows the comparision of different models using AP (Average Precision) as the metric. 

%Here is the performance of three models using AP (Average Precision) as the metric. (i) Mask-RCNN : $39.8$ (ii) Mask-RCNN (backpropagate over captions): $40.5$ (iii) Mask-RCNN (backpropagate over captions, tags): $40.9$. 



\begin{figure}[t]
	\centering
	\subfigure{\includegraphics[width=\linewidth, height=0.7\linewidth]{./figures/instance-seg-captions-tags-proposed-arch.pdf}}
	\caption{Our framework, for instance segmentation with multiple types of auxiliary information simultaneously.  Mask-RCNN is used for instance segmentation. LSTM based caption generator to use textual descriptions of an image and a multiclass image classifier to use image level tags both at the test time. }
	% Note that BB refers to bounding box.}
	\label{fig:instance-seg-captions-tags-proposed-arch}
\end{figure}

\subsection{Image Captioning given Image Level Tags}

We have conducted experiments on the MS COCO dataset with image caption prediction as the primary task and image tags as the auxiliary task. Figure~\ref{fig:caption-tags-proposed-arch} describes our proposed MTL architecture in detail. The base architecture was ``Show, Attend and Tell''(SAT)~\cite{xu2015show}, one of the prominent image captioning model.  To use image level tags, we branch off after the encoder module and design a multi-class classifier. The resultant feature map is passed through an average pooling layer, a fully connected layer, and then finally a sigmoid activation function to get probabilty for each of the 80 classes. Using BLEU-4 as the metric, performances are: (i) SAT: 25.8 (ii) SAT (multi-task): 27.4 (iii) SAT (multi-task + backpropagate over tags): 29.6. We also gain on other metrics such as ROUGE and CIDEr.

\setlength{\tabcolsep}{7pt}
\begin{table}[t]
	   \centering
	   \begin{tabular}{lcccc}
	       \toprule[1.5pt]
	       \textbf{} & \textbf{Mask} & \textbf{Mask-BP-C-ES} & \textbf{Mask-BP-CT-ES}\\
	       \midrule
	       AP & 39.8 &  40.5  & 40.9  \\       
	       \bottomrule[1.5pt]
	   \end{tabular}
	   \caption{Comparison of results for instance segmentation with captions and tags as auxiliary information. Mask represent baseline pretrained network. Mask-BP-C-ES refers to backpropagation over captions and Mask-BP-CT-ES refers to  backpropagation over captions and tags.}
	   \label{table:instance_segmentation_caption_tags_comparison}
	\end{table}



\subsection{Image Captioning given Image Level Tags}

We have conducted experiments on the MS COCO dataset with image caption prediction as the primary task and image tags as the auxiliary task. 
Figure~\ref{fig:caption-tags-proposed-arch} describes our proposed MTL architecture in detail. 
The base architecture was ``Show, Attend and Tell''(SAT)~\cite{xu2015show}, one of the prominent image captioning model.  To use image level tags, we branch off after the encoder module and design a multi-class classifier. The resultant feature map is passed through an average pooling layer, a fully connected layer, and then finally a sigmoid activation function to get probabilty for each of the 80 classes. Using BLEU-4 as the metric, comparision results are shown in Table~\ref{table:image_captioning_comparison}.

\begin{figure}[t]
	\centering
	\subfigure{\includegraphics[width=\linewidth]{./figures/caption-tags-proposed-arch.pdf}}
	\caption{Our framework for image captioning using ``Show, Attend and Tell''(SAT)~\cite{xu2015show} and a multiclass image classifier to use image level tags at the test time.}
	% Note that BB refers to bounding box.}
	\label{fig:caption-tags-proposed-arch}
\end{figure}

\subsection{Multimodal DNNs}

\setlength{\tabcolsep}{7pt}
\begin{table}[t]
	   \centering
	   \begin{tabular}{lcccc}
	       \toprule[1.5pt]
	       \textbf{} & \textbf{SAT} & \textbf{SAT-MT} & \textbf{SAT-ES}\\
	       \midrule
	       BLEU-4 & 25.8 &  27.4  & 29.6 \\       
	       \bottomrule[1.5pt]
	   \end{tabular}
	   \caption{Comparison of results for image captioning. SAT and SAT-MT represent baseline pretrained network and baseline trained with MTL strategy respectively. We refer to our approach as SAT-BP-ES, here ES stands for early stopping as a regularizer during prediction.}
	   \label{table:image_captioning_comparison}
	\end{table}

We have also done experiments with baseline models using auxiliary information as input, but our approach performs better them. 
In the case of semantic segmentation, we have designed a model
based on DeepLabv3+, which takes multi-hot encoding representation
of image-level tags as input. Our model combines
intermediated representation of images generated by
DeepLabv3 with the multi-hot representation of tags. Let’s
say dimension of image features are $a \times b \times c$ and tag representation is a vector of size $20$, we have first broadcasted the
tag vector to every position in height and width, and the resulting
feature dimension becomes $a\times b \times (c+20)$. Then we pass the features through a $1\times1$ convolution to make the resulting dimension as $a \times b \times c$ again. The rest of the network is same as DeepLabv3+. Compared to baseline DeepLab for semantic segmentation with an MIoU $82.59$, using tags as input only improves it to $84.21$, compared to our framework which gives an MIoU of $86.01$ using the same information. We also tried inputting caption embeddding generated using ``InferSent''~\cite{conneau2017supervised} from Facebook AI Research, to the Mask-RCNN. However, in this case, our training did not converge. This highlights the advantage with our framework which allows the primary task to be trained separately first, and then fine-tune the joint model in an efficient manner.  Further, we note that multi-task training does not require any commonly annotated dataset unlike when auxiliary information is given as input.  Further, our framework does not requires any commonly annotated dataset unlike the approaches which take auxiliary information as input. 
>>>>>>> be51db20267327e88e3d2e1b2153be0d98f315ee


==> sections/results_semantic_seg_bak.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{./figures/sem-seg-proposed-arch.pdf}
	\caption{Our architecture for semantic segmentation using image level tags as test time evidence.}
	\label{fig:proposed-sem-seg-arch}
\end{figure}

\subsection{Semantic Segmentation}
\label{sec:semantic_seg}

The task of semantic segmentation involves assigning a label to each pixel in the image from a fixed set of object categories. Semantic segmentation is an important part of scene understanding and is critical first step in many computer vision tasks. In many semantic segmentation applications, image level tags are often easily available and encapsulate important information about the context, scale and saliency. We explore the use of such tags as auxiliary information at test time for improving the prediction accuracy. As clarified in earlier sections as well, though using auxiliary information in the form of natural language sentences \cite{hu2016segmentation, liu2017recurrent} have been suggested, these earlier works have used this information only during the training time. This is unlike us where we are interested in exploiting this information both during training as well as test.

\myparagraph{Evaluation Dataset}
%
For evaluation, we use PASCAL VOC 2012 segmentation benchmark \cite{everingham2010pascal}. It consists of 20 foreground object classes and one background class. We further augmented the training data with additional segmentation annotations provided by Hariharan et al.~\cite{hariharan2011semantic}. The dataset contains 10582 training and 1449 validation images. We use mean intersection over union (mIOU) as our evaluation metric which is a standard for segmentation tasks. 

\myparagraph{Our Implementation}
%
Our implementation builds on the publicly available official implementation of DeepLabv3+ \cite{chen2018encoder} available at \cite{deeplab-code}. For ease of notation, we will refer the DeepLabv3+ model as `DeepLab'. To use our framework, we have extended the DeepLab architecture to simultaneously solve the classification task in an MTL setting. Figure \ref{fig:proposed-sem-seg-arch} describes our MTL architecture. Starting with the original DeepLab architecture (top part in the figure), we branch off after the encoder module to solve the classification task. The resultant feature map is passed through an average pooling layer, a fully connected layer, and then finally a sigmoid activation function to get probabilty for each of the 20 classes (background class is excluded). 

For training, we make use of cross-entropy based loss, for the primary and binary cross entropy loss for the secondary task. We first train the segmentation only network to get the initial set of weights. These are then used to initialize the weights in the MTL based architecture (for the segmentation branch). The weights in the classification branch are randomly initialized. This is followed by a joint training of the MTL architecture. During prediction time, for each image, we back-propagate the binary cross entropy loss based on observed evidence over the auxiliary task (for test image) resulting in weights re-adjusted to fit the evidence. These weights are used to make the final prediction (per-image). The parameters in our experiments were set as follows. During training, the $\lambda$ parameter controlling the relative weights of the two losses is set of $1$ in all our experiments. During prediction, number of early stopping iterations was set to $2$. $\alpha$ parameter for weighing the two norm regularizer was set to $1$. We have used SGD optimizer with learning rate of $7* 10^{-4}$ at test time. 

\myparagraph{Compared Models}
%
The table on the right compares the performance of our approach with various approaches. 
\setlength{\columnsep}{5pt}%
\setlength{\intextsep}{5pt}%
\setlength{\tabcolsep}{2pt}
\begin{wraptable}{r}{0.5\linewidth}
	\centering
	\begin{tabular}{lcc}
		\toprule[1.5pt]
		\multirow{2}{*}{\multilineC{\bf Method}} & \multicolumn{2}{c}{\bf mIoU} \\  \cmidrule{2-3} & { No-MS} & {MS} \\ 
		\toprule[1.5pt]
		DL       & 82.45 & 83.58  \\
		DL-MT    & 82.59 & 83.55  \\
		DL-Pr    & 84.47 & 85.29  \\
		MM       & 83.66 & 85.12  \\
		\midrule
		Ours(L2) & 85.97 & 86.88  \\
		Ours(ES) & 86.01 & 86.84  \\
		%		DL-BP-L2-Pr & 86.10& 87.00     \\
		%		DL-BP-ES-Pr & \textbf{86.22} & \textbf{87.03}    \\
		\bottomrule[1.5pt]
	\end{tabular}
\end{wraptable}

\setlength\arrayrulewidth{1.25pt}
% \begin{wraptable}{r}{0.45\linewidth}
% \begin{tabular}{|*{3}{l|cc|}} 
% \cline{1-3}
% \multirow{2}{*}{\multilineC{\bf Method}} & \multicolumn{2}{c|}{\bf mIoU} \\
% \cline{2-3} & { No-MS} & {MS} \\
% \cline{1-3}
% DL       & 82.45 & 83.58  \\
% DL-MT    & 82.59 & 83.55  \\
% DL-Pr    & 84.47 & 85.29  \\
% MM       & 83.66 & 85.12  \\
% \cline{1-3}
% Ours(L2) & 85.97 & 86.88  \\
% Ours(ES) & 86.01 & 86.84  \\
% %		DL-BP-L2-Pr & 86.10& 87.00     \\
% %		DL-BP-ES-Pr & \textbf{86.22} & \textbf{87.03}    \\

% \cline{1-3}
% \end{tabular}

% \end{wraptable}



The model `DL' uses vanilla DeepLab based architecture, whereas `DL-MT' is trained using the MTL framework but do not use the evidence at the test time. One of our naive alternative is to simply prune or zero the probability of the label at each pixel which is not present in the tag set. The suffix `Pr' to refers to such alternative. We have also designed our own multi-modal network, referred to as MM, which takes RGB image and image lebels as input.
Our designed for MM takes inspiration from \cite{rosenfeld2018priming} but somewhat more sophisticated than it. We take image features of size $a \times b \times c$ at an intermediate layer as shown in Figure~\ref{fig:proposed-sem-seg-arch} and then broadcast the
one-hot encoding of image labels which is of size 20 to every position in height and width. The resulting features dimensions become $a\times b \times (c+20)$, which are than pass through a $1\times1$ convolution to make the resulting dimension as $a \times b \times c$ again. The rest of the network is the same as DeepLabv3+. We also note that \cite{rosenfeld2018priming} report less than $1\%$ of improvements on a older version of dataset as compared to ours $3.9\%$.

We experiment with two variations of our approach based on the choice of regularizer during prediction: ES uses early stopping and L2 uses an L2-norm based penalty. Original DeepLab paper~\cite{chen2018encoder}  also experiments with inputting images at multiple scales i.e, \{$0.5$,$0.75$,$1.0$,$1.25$,$1.5$\} as well as using left-right flipped input images, and then taking a mean of the predictions. We refer to this as multi-scaling (MS) based approach. We compare each of our models with multi-scaling being on and off in our experiments.

\input{./sections/table-sem-seg-classwise-miou.tex}

\myparagraph{Quantitative Results}
%
Table~\ref{table:seg_obj_comparision} presents the results for each of the object categories. For all the object categories except two, we perform better than the baselines. The gain is as high as 10 points (or more) for some of the classes. 

\myparagraph{Impact of Noise} 
The table on the right examines the performance of various approaches in the presence of noisy evidence. 
%\begin{comment}
\setlength{\columnsep}{5pt}%
\setlength{\intextsep}{5pt}%
\setlength{\tabcolsep}{4pt}
\begin{wraptable}{r}{0.65\linewidth}
	\centering
	\begin{tabular}{lcccc}
		\toprule[1.5pt]
		\textbf{Model} & \multicolumn{4}{c}{\textbf{\# of noisy tags ($k$)}} \\
		\midrule
		& \textbf{0}   & \textbf{1}   & \textbf{2}   & \textbf{3}     \\
		\midrule
		Ours & 86.0 & 85.3  &  84.0 & 83.4         \\
		Pruning  & 84.5 & 83.9  & 82.5 & 82.2 \\
		MM       & 83.7 & 83.7  & 83.4  & 83.2 \\
		\bottomrule[1.5pt]   
	\end{tabular}
\end{wraptable}
%\end{comment}
For each image we randomly introduce $k$ (for varying values of $k$) additional (noisy) tags which were not part of the original set\footnote{This experiment was done without using multi-scaling}. Our approach is fairly robust to such noise, and its performance degrades slowly with increasing amount of noise. Even when we have 3 additional noisy tags added, we still do better than baseline DeepLab model with a performance of 82.59.

\begin{figure}[t]
	\centering
	\subfigure{\includegraphics[width=\linewidth]{./figures/sem-seg-vis-output_main.pdf}}
	\caption{Comparison of visual results on semantic segmentation using image level tags as the test time auxiliary information.}
	\label{fig:sem-seg-vis-output-main}
\end{figure}

\myparagraph{Visual Results}
%
Figure \ref{fig:sem-seg-vis-output-main} show the visual comparison of results for a set of hand picked examples. We note that our model is not only able to enhance the segmentation quality of already discovered objects, it is also able to discover new objects which are completely missed by the baseline. We show more results in the supplementary material.

\myparagraph{Inference Time}
%
Inference time on one image for different models are: $0.15$ seconds for DeepLab, $2.6$ seconds for Deeplab with multi-scaling, and $1.4$ seconds for our model with early stopping of 2 back-propagation. Our model with multi-scaling takes $3.85$ seconds on a GTX 1080 Ti GPU. 
%
\begin{figure}[t]
	\centering
	\subfigure{\includegraphics[height=0.35\linewidth]{./figures/mIoU_vs_backprop.pdf}} \;
	\subfigure{\includegraphics[height=0.35\linewidth]{./figures/mIoU_vs_reg.pdf}}		
	\caption{Sensitivity of results on number of back-propagation iterations (early stopping) and $\alpha$ parameter (L2-norm)}
	\label{fig:sem-seg-sensitivity}	
\end{figure}

\myparagraph{Ablation Study}
%
Figure \ref{fig:sem-seg-sensitivity} presents the sensitivity analysis with respect to the number of early stopping iterations (left) and the parameter controlling the weight of the L2 regularizer during prediction (right). There is a large range of values where we get significant improvements. 


